Real-Time Analytics by Coordinating Reuse and Work Sharing

Analytical tools often require real-time responses for highly concurrent parameterized workloads. A common solution is to answer queries using materialized subexpressions, hence reducing processing at runtime. However, as queries are still processed individually, concurrent outstanding computations accumulate and increase response times. By contrast, shared execution mitigates the effect of concurrency and improves scalability by exploiting overlapping work between queries but does so using heavyweight shared operators that result in high response times. Thus, on their own, both reuse and work sharing fail to provide real-time responses for large batches. Furthermore, naively combining the two approaches is ineffective and can deteriorate performance due to increased filtering costs, reduced marginal benefits, and lower reusability. In this work, we present ParCuR, a framework that harmonizes reuse with work sharing. ParCuR adapts reuse to work sharing in four aspects: i) to reduce filtering costs, it builds access methods on materialized results, ii) to resolve the conflict between benefits from work sharing and materialization, it introduces a sharing-aware materialization policy, iii) to incorporate reuse into sharing-aware optimization, it introduces a two-phase optimization strategy, and iv) to improve reusability and to avoid performance cliffs when queries are partially covered, especially during workload shifts, it combines partial reuse with data clustering based on historical batches. ParCuR outperforms a state-of-the-art work-sharing database by 6.4x and 2x in the SSB and TPC-H benchmarks respectively

==> parcur/algorithms/reuse-phase.tex <==
\begin{algorithm}
\SetAlgoLined
\caption{Reuse Optimization Phase}
\label{parcur:alg:reuse-phase}
\SetKwProg{Fn}{Function}{ :}{}
\Fn{REUSE\_OPT($plan$)}{
\If {$plan.hasConverged()$}{
    $res = \textcolor{blue}{REUSE\_OPT\_REC}(plan.root)$ \;
    $plan = REWRITE(plan, res.rewrites)$ \;
}
}
\Return $plan$ \;

\Fn{\textcolor{blue}{REUSE\_OPT\_REC}($cur$)}{ \label{line:reuse-phase-rec}
$covered=false$; $dcost=0.0$; $cut = null$ \;
$rewrites = \emptyset$ \;
\If {$cur.next \neq null\ and\ cur.div \neq null$} {
    $rnext=\textcolor{blue}{REUSE\_OPT\_REC}(cur.next)$ \;
    $rdiv=\textcolor{blue}{REUSE\_OPT\_REC}(cur.div)$ \;
    $covered=true$ \;
    $merge = (rnext.covered\ or\ rnext.cut \neq null)\ and\
        (rdiv.covered\ or\ rdiv.cut \neq null)$ \;
    \If {$rnext.covered = false$} {
        $covered=false$ \;
        $dcost = rnext.dcost + cur.cost$ \;
        $benefit = dcost - rnext.cut.dcost - rnext.cut.fcost$ \;
        $cut = rnext.cut$ \;
        \If {$rnext.cut \neq \emptyset\ and\  benefit > 0$} {
            $rewrites = rewrites \cup \{ cut \}$ \;
            $rnext.cut.set = \emptyset$ \;
            $dcost = 0.0$ \;
            $covered = true$ \;
        }
        \If {$merge\ and\ rnext.cut.set \neq \emptyset$} {
            $cut = rnext.cut$
        }
    }
    \If {$dnext.covered = false$} {
        $dcost = dnext.dcost$ \;
        $covered=false$ \;
        \If {$merge\ and\ dnext.cut.set \neq \emptyset$} {
            $cut = merge(cut, rdiv.cut)$
        }
    }
    \If {$covered = false$} {
        $benefit = dcost - cut.dcost - cut.fcost$ \;
        \If {$cut \neq \emptyset\ and\  benefit > 0$} {
            $rewrites = rewrites \cup \{ cut \}$ \;
            $cut.set = \emptyset$ \;
            $dcost = 0.0$ \;
            $covered = true$ \;
        }
    }
}
\ElseIf {$cur.next \neq null$} {
    $rnext=\textcolor{blue}{REUSE\_OPT\_REC}(cur.next)$ \;
    $rewrites = rewrites \cup rnext.rewrites$ \;
    $covered=rnext.covered$ \;
    \If {$is\_covered = false$} {
        $dcost = rnext.dcost + cur.cost$ \;
        $benefit = dcost - rnext.cut.dcost - rnext.cut.fcost$ \;
        $cut = rnext.cut$ \;
        \If {$benefit > 0$} {
            $rewrites = rewrites \cup \{ cut \}$ \;
            $cut = CUT(\emptyset, cut.dcost, cut.fcost)$ \;
            $covered = true$ \;
        }
    }
}
\If {$covered=false\ and\ cur.reusable = true$} {
    \If {$cut.set = \emptyset\ or\
    cut.dcost + cut.fcost - cur.dcost > dcost$} {
        $cut = CUT(\{cur, dcost, cur.fcost)$
    }
}
}
\Return $RES(covered, rewrites, cut)$ \;

\end{algorithm}

==> parcur/algorithms/reuse-phase2.tex <==
\begin{algorithm}
\SetAlgoLined
\caption{Reuse Optimization Phase}
\label{parcur:alg:reuse-phase}
\SetKwProg{Fn}{Function}{ :}{}
\Fn{REUSE\_OPT($plan$)}{
\If {$plan.hasConverged()$}{
    $res = \textcolor{blue}{REUSE\_OPT\_REC}(plan.root)$ \;
    $plan = REWRITE(plan, res.rewrites)$ \;
}
}
\Return $plan$ \;

\Fn{\textcolor{blue}{REUSE\_OPT\_REC}($cur$)}{
    \label{line:reuse-phase-rec}
    \If {$!cur$} {
        \Return $null$ \;
    }
    $covered=false$; $dcost=0$; $rewrites = \emptyset$ \;
    $cut = CUT(\emptyset, 0, 0)$ \;
    $rnxt=\textcolor{blue}{REUSE\_OPT\_REC}(cur.next)$ \;
    $rdiv=\textcolor{blue}{REUSE\_OPT\_REC}(cur.div)$ \;
    \COMMENT {/* Make super-cut if cut exists on both sides */ } \;
    $merge =\ !rnxt \ \&\&\ !rdiv$ \;
    $merge\ \&\&= (rnxt.cut.set \neq \emptyset\ ||\ rnxt.covered)$ \;
    $merge\ \&\&= (rdiv.cut.set \neq \emptyset\ ||\ rdiv.covered)$ \;
    \If {$!rnxt$} {
        $covered=rnxt.covered$ \;
        $rewrites = rewrites \cup rnxt.rewrites$ \;
        \COMMENT {/* Next has downstream operators so far */ } \;
        \If {$!rnxt.covered$} {
            $dcost = rnxt.dcost + cur.cost$ \;
            $gain = dcost \text{-} rnxt.cut.dcost \text{-} rnxt.cut.fcost$ \;
            $cut = rnxt.cut$ \;
            \COMMENT {/* Reuse cut for next */ } \;
            \If {$ cut.set \neq \emptyset\ \&\&\  gain > 0$} {
                $rewrites = rewrites \cup \{ cut \}$ \;
                $cut = CUT(\emptyset, 0, 0)$ \;
                $dcost = 0$ \;
                $covered = true$ \;
            }
            \COMMENT {/* Merge to super-cut */ } \;
            \If {$merge\ \&\&\ rnxt.cut.set \neq \emptyset$} {
                $cut = rnxt.cut$
            }
        }
    }
    \If {$!rdiv$} {
        $rewrites = rewrites \cup rdiv.rewrites$ \;
        \COMMENT {/* Div has downstream operators so far */ } \;
        \If {$!rdiv.covered$} {
            $dcost = dcost + rdiv.dcost$ \;
            $covered=false$ \;
            \If {$merge\ \&\&\ rdiv.cut.set \neq \emptyset$} {
                $cut = MERGE\_CUT(cut, rdiv.cut)$
            }
        }
        \If {$!covered$} {
            $gain = dcost - cut.dcost - cut.fcost$ \;
            \COMMENT {/* Reuse merged cut */ } \;
            \If {$cut.set \neq \emptyset\ \&\&\  benefit > 0$} {
                $rewrites = rewrites \cup \{ cut \}$ \;
                $cut = CUT(\emptyset, cut.dcost, cut.fcost)$ \;
                $dcost = 0.0$ \;
                $covered = true$ \;
            }
        }
    }
    \If {$!covered\ \&\&\ cur.reusable$} {
        $ccost = cut.dcost + cut.fcost - cur.dcost$ \;
        \If {$cut.set = \emptyset\ ||\ ccost > dcost$} {
            $cut = CUT(\{cur\}, dcost, cur.fcost)$
        }
    }
}
\Return $RES(covered, rewrites, cut, dcost)$ \;

\end{algorithm}

==> parcur/txt/architecture.tex <==
\section{System Architecture}

We present \system: a system for processing a large number of concurrent short-running queries. By using a data partitioning and a cache that is optimized for the workload, \system\ permits the creation of multiple access paths that specialize execution to each data region and provide different opportunities for reducing processing time: (i) avoid recurring computations, and (ii) decrease the cost of data access. During optimization and execution, \system\ selects the most beneficial access path for each part of the data, and adaptively shares work to bound latency.


\begin{figure}[t]
 \centering
	\includegraphics[width=0.75\hsize]{../figures/architecture.pdf}
 \vspace{-4mm}
	\caption{Architecture of \system.}
	\label{parcur:fig:architecture}
 \vspace{-4mm}
\end{figure}

Figure \ref{parcur:fig:architecture} depicts an overview of the architecture. There are two main components: (i) the \emph{tuner}, and (ii) the \emph{executor}. Both components are workload-dependent and adaptive; incoming queries trigger execution, and at the same time drive tuning. The tuner analyzes the incoming queries, and adapts the system's state to workload-shifts by sporadically changing the available access paths: (i) new sub-queries are materialized, whereas others are deleted, (ii) the data layout changes; data is re-partitioned and new access methods become available. Then, given the data partitioning and the cache, the executor processes a query batch, and by adaptively selecting access paths and by sharing work at the level of fine-grained partitions, it minimizes response time.

Decoupling the tuner and the executor happens for two reasons: (i) to reduce  overheads and (ii) to ensure that tuning will pay off. Tuning requires solving the caching and the data-layout optimization problems, both of which have large search-spaces, and involve multiple costly passes over the full data. On the one hand, we require query execution to be interactive, and thus we cannot tune the data layout and the caches in the critical path: the overhead would be excessive. On the other hand, the investment of tuning at runtime may not pay off even in a high concurrency setup, and larger query sequences (across batches) may be needed to amortize the cost.

%Decoupling the tuner and the executor happens for two reasons: (i) to reduce  overheads and (ii) to ensure that tuning will pay off. Tuning requires solving the view-selection and the data-layout optimization problems, both of which are NP-hard \cite{gupta1997selection,sun2016skipping}, and involve costly data move operations. On the one hand, we require query execution to be interactive, and thus we cannot inject physical design tuning in the critical path: the overhead would be excessive. On the other hand, the investment of changing the physical design at runtime may not payoff even in a high concurrency system, and larger query sequences (across batches) may be needed to amortize the cost.

Despite being decoupled, both subsystems are conscious to each other, and the behavior of the one affects the behavior of the other. In order to efficiently execute the workload, the executor takes advantage of the structures that the tuner has created, and the tuner should be aware of the shared execution costs in order to materialize the most appropriate sub-queries. 

%For example, it uses data skipping to only process the queries that are relevant for each partition, or it avoids redundant computations by injecting materialized views in the query plans. The tuner, in its turn, chooses to materialize a set of views that minimizes the cost of batch processing. Thus, the tuner should be aware of the employed shared workload optimization algorithm and of the impact of view-selection on execution.


==> parcur/txt/experiments.tex <==
\section{Experimental Evaluation}
\label{parcur:sec:evaluation}

\begin{figure*}[h]
\begin{tabular}{@{}l@{}l@{}l}
\begin{minipage}{0.33\hsize}
    \centering\includegraphics[width=14pc]{../figures/cor01_part.pdf}\\
        \centering {\footnotesize(a) selectivity 0.1\%}
        \end{minipage}
        &
    \begin{minipage}{0.33\hsize}
\centering\includegraphics[width=14pc]{../figures/cor1_part.pdf}\\
    \centering {\footnotesize(b) selectivity 1\%}
    \end{minipage}
    &
    \begin{minipage}{0.33\hsize}
\centering\includegraphics[width=14pc]{../figures/cor10_part.pdf}\\
    \centering {\footnotesize(c) selectivity 10\%}
    \end{minipage}
\end{tabular}
\caption{\label{parcur:fig:qdpartitioning} Impact of partitioning when a correlated workload and various selectivities and batch sizes are used.}
\end{figure*}

This section experimentally evaluates \system\ and shows how the physical design can help us significantly outperform state-of-the-art work-sharing approaches and achieve a lower query batch response time in concurrent selective workloads. More specifically, we investigate in which cases we can take advantage of the data layout, in which cases of the views and when we need both. To this end, we present a suite of micro-benchmarks that assess various aspects of the design space and showcase the strengths of the proposed framework.

\textbf{Dataset}. We use the TPC-DS dataset in scale factor $10$. Specifically, as at the moment the physical design optimization process of \system\ only considers star-schemas, we use the \texttt{\Verb"store\_sales"} fact table along with the corresponding dimension tables.

\textbf{Workload}. We generate random SPJ queries over the defined schema. The dimensions that affect performance and based on which we parameterize the workloads are: (i) \emph{concurrency}, (ii) \emph{selectivity on the fact table}, (iii) \emph{the number of query templates per batch}\footnote{With the term query template we refer to the different join combinations that appear in a batch}, and (iv) the \emph{correlation pattern}. The latter indicates whether the queries of a batch target the same regions of the fact table. More specifically, we consider three classes of workloads based on the correlation pattern:
\begin{itemize}
    \item \emph{correlated workloads}: All queries of a batch have the same filters on the fact table. This class represents cases where a data region can temporarily become extremely hot and popular.
    \item \emph{uncorrelated workloads}: There are no locality patterns and each query has a random filter on the fact table.
    \item \emph{semi-correlated workloads}: The workload is partitioned into disjoint groups of queries where all queries of a group share the same filters on the fact table. This simulates multiple hot regions in the dataset.
\end{itemize}
Note that as we have found the selectivity and the correlation pattern on the dimension tables to play a minor role, for all the experiments and dimension tables, we consider an uncorrelated access pattern and a selectivity of $20\%$. Henceforth, with the term selectivity we abusively refer to the selectivity on \texttt{\Verb"store\_sales"}.

\textbf{Algorithms}. We compare \system\ against the baseline of \roulette. \roulette\ is a state-of-the-art work-sharing system, but which is oblivious to both the data layout and the possibly available materialized views.

\textbf{Hardware}. All experiments took place on a single server that features an Intel(R) Xeon(R) Gold 5118 CPU @ 2.30GHz with $2$ sockets, $12(\times2)$ threads per socket, $376$GB of DRAM, $32$KB L1 cache, $1$MB L2 cache and $16$MB L3 cache. All experiments took place in memory, in a single NUMA node.

\textcolor{red}{TODO: Remove data layout experiments}

\subsection{Impact of Data Layout}

First, we evaluate the impact of partitioned execution. In contrast to \roulette\, that optimizes and executes the whole fact table as a single partition, \system\ uses a Qd-tree to partition and re-organize the dataset and then optimization and execution happen in a per partition level.

\begin{figure}[h]
\begin{tabular}{@{}l@{}l}
\begin{minipage}{0.5\hsize}
    \centering\includegraphics[width=10pc]{../figures/cor_small.pdf}\\
        \centering {\footnotesize(a) correlated workload}
        \end{minipage}
        &
    \begin{minipage}{0.5\hsize}
\centering\includegraphics[width=10pc]{../figures/uncor_small.pdf}\\
    \centering {\footnotesize(b) uncorrelated workload}
    \end{minipage}
\end{tabular}
\caption{\label{parcur:fig:corvsuncor} Impact of partitioning on correlated and uncorrelated workloads of selectivity $1\%$.}
\end{figure}

\subsubsection{Selectivity and correlation pattern}

In these experiments, we evaluate how partitioned execution can take advantage of the selectivity and the correlation pattern. We test two workloads: a correlated and an uncorrelated one. In both workloads, there are no available views and we vary the query batch size and the selectivity on the \texttt{\Verb"store\_sales"} table. 

Figure \ref{parcur:fig:corvsuncor} depicts the differences between the correlated and uncorrelated workloads for a selectivity $1\%$. The bars indicate the total execution time of each system, whereas the lines show the corresponding join and aggregation time. The portion of the bars that is above the lines corresponds to scanning and filtering. We observe that partitioning favors correlated workloads, where it provides an average speedup of $2.2\times$. Intuitively, partitioning can be useful during scanning as it allows to skip blocks, whereas during join the same computations will be always performed regardless of whether the data is partitioned. Thus, the merits of \system, when there are no views available, are highlighted in \emph{scan-heavy} workloads and fade out in \emph{join-heavy} ones. 

In Figure \ref{parcur:fig:qdpartitioning}, we use correlated workloads and this time we vary the selectivity. Conclusions are similar: the lower the selectivity, the more scan-heavy the workload, the higher the benefit for \system. As \system\ allows aggressive data skipping, in low selectivities execution is always bound by the cost of join and aggregation. In contrast, in \roulette, the scan and filtering time dominates execution for small selectivities, and the bottleneck gradually shifts to join as selectivity increases. 

\begin{figure}[h]
 \centering
	\includegraphics[width=0.8\hsize]{../figures/cor_filters.pdf}	
	\caption{Impact of the number of filtering attributes for a correlated workload of $1\%$ selectivity.}
	\label{parcur:fig:filters}
\end{figure}

\textbf{Takeaway:} By using the optimized data layout, our adaptive executor achieves its goal and accelerates concurrent selective workloads. In general, we identify a design space where the various options depend on whether the workload is scan- or join-heavy. Partitioning by itself favors scan-heavy queries.

% When there are no views, \system\ is especially favored by selective workloads. Moreover, the more scan-heavy the workload, the highest the benefit that \system\ offers.

\begin{figure*}[h]
\begin{tabular}{@{}l@{}l@{}l}
\begin{minipage}{0.33\hsize}
    \centering\includegraphics[width=14pc]{../figures/cor1_views.pdf}\\
        \centering {\footnotesize(a) selectivity 1\%, 3 templates}
        \end{minipage}
        &
    \begin{minipage}{0.33\hsize}
\centering\includegraphics[width=14pc]{../figures/cor10_views.pdf}\\
    \centering {\footnotesize(b) selectivity 10\%, 3 templates}
    \end{minipage}
    &
    \begin{minipage}{0.33\hsize}
\centering\includegraphics[width=14pc]{../figures/cor_templates.pdf}\\
    \centering {\footnotesize(c) 512 queries}
    \end{minipage}
\end{tabular}
\caption{\label{parcur:fig:views-cor} Impact of concurrency and selectivity on correlated workloads.}
\end{figure*}
\begin{figure*}[h]
\begin{tabular}{@{}l@{}l@{}l}
\begin{minipage}{0.33\hsize}
    \centering\includegraphics[width=14pc]{../figures/uncor1_views.pdf}\\
        \centering {\footnotesize(a) selectivity 1\%, 3 templates}
        \end{minipage}
        &
    \begin{minipage}{0.33\hsize}
\centering\includegraphics[width=14pc]{../figures/uncor10_views.pdf}\\
    \centering {\footnotesize(b) selectivity 10\%, 3 templates}
    \end{minipage}
    &
    \begin{minipage}{0.33\hsize}
\centering\includegraphics[width=14pc]{../figures/uncor_templates.pdf}\\
    \centering {\footnotesize(c) 512 queries}
    \end{minipage}
\end{tabular}
\caption{\label{parcur:fig:views-uncor} Impact of concurrency and selectivity on uncorrelated workloads.}
\end{figure*}

\subsubsection{Multiple filters on the fact table}

In the previous experiments, we evaluate a single filter over the fact table. In reality, we may have compound filters on multiple attributes. As the evaluation of multiple filters on \texttt{\Verb"store\_sales"} will render the scan and filtering phase more expensive, we expect it to increase the benefits of \system. We repeat the previous experiment for the scan-heavy correlated workload, but this time we compute over the fact table five filters of joint selectivity $1\%$. Figure \ref{parcur:fig:filters} depicts the results. We observe that the average speedup of \system\ over \roulette\  increases from $2.65\times$ to only $3.1\times$. The reason for this is the RL algorithm that both systems employ. By adaptively reordering the filtering operators, the optimization algorithm learns the selectivity of each filter, computes them in increasing order of selectivity and eagerly prunes intermediate results before all five filters are evaluated.

\textbf{Takeaway:} For selective workloads, the number of filters has minimal impact on performance.

\subsubsection{Workload shift}

Finally, we assess how both systems respond to workload shifts. We assume a batch of $512$ queries of selectivity $1\%$ and a fine-grained partitioning of the dataset. Initially, the workload is correlated and all queries target the same range of the fact table. Then, we assume that a second partition is becoming hot and $256$ queries migrate to the second partition (semi-correlated workload). Then, the workload further spreads, and now we have $4$ hot partitions with $128$ queries each etc. Figure \ref{parcur:fig:partitioningshift} shows the results. In the beginning, \system\ is $4.7\times$ faster than the scan-bound \roulette. Once again, as a larger fraction of the fact table is processed, the bottleneck shifts from scan/filtering to join/aggregation and the difference between the two system diminishes. However, even when the workload has spread enough and spans the $64\%$ of the fact table, \system\ is still $2.6\times$ faster than \roulette. We notice that as we access more partitions, the difference in the scan/filtering time decreases, whereas the difference in join/aggregation increases. On the one hand, as \roulette\ always scans the whole dataset, the scan/filtering time is near constant\footnote{As \roulette\ has not an optimized layout, records are filtered in a random order that leads to increased branch misprediction, which in turn slightly increases the scan/filtering time.}, while \system{}'s scan time increases as it can skip less and less blocks. On the other hand, the semi-correlated workload helps \system\ to specialize execution and apply more efficient aggregation in the  partition level. For the case of the $64$ partitions, \system\ processes only $8$ queries per partition, whereas \roulette\ $512$. The lenghts of the bitmasks that are used for the corresponding query-set operations at this point yield a significant performance difference.

\begin{figure}[h]
\begin{tabular}{@{}l@{}l}
\begin{minipage}{0.5\hsize}
    \centering\includegraphics[width=10pc]{../figures/parti-shift-roulette.pdf}\\
        \centering {\footnotesize(a) \roulette}
        \end{minipage}
        &
    \begin{minipage}{0.5\hsize}
\centering\includegraphics[width=10pc]{../figures/part-shift-parkour.pdf}\\
    \centering {\footnotesize(b) \system}
    \end{minipage}
\end{tabular}
\caption{\label{parcur:fig:partitioningshift} Robustness of partitioning to workload shift.}
\end{figure}

\textbf{Takeaway:} By specializing execution to each partition, \system\ reduces the total aggregation cost and becomes robust to shifts among semi-correlated workloads.

\subsection{Impact of Views}

Thus far, we have seen that by only using data layout optimization, \system\ mainly favors scan-heavy correlated workloads. In this section, we will see that by pruning joins, the use of materialized views renders it also suitable for uncorrelated and semi-correlated join-heavy use cases. Surprisingly though, views cannot be used efficiently by themselves and layout optimization is always needed. To select the most appropriate view per partition, \system\ employs the RL algorithm of Section \ref{parcur:sec:learning}.

\subsubsection{Selectivity and correlation pattern}

\textcolor{red}{TODO: Present experiments wrt layout.}

\textcolor{red}{TODO: Evaluate VSWO}

\textcolor{red}{TODO: Evaluate materialization algorithm}

Figures \ref{parcur:fig:views-cor} and \ref{parcur:fig:views-uncor} show the impact of views for various batch sizes and selectivities for a correlated and an uncorrelated workload. We evaluate three versions of \system\ against the baseline of \roulette: (i) \emph{\system\ (no partitioning)} signifies that we use views, but no layout optimization and execution takes place in a single partition, (ii) \emph{\system\ (no views)} is the version of \system\ that we evaluated in the previous section, i.e., partitioning is enabled but there are no views available, and (iii) \system\ is the full version of our system.

The first observation is that \emph{\system\ (no partitioning)} is almost always slower than the baseline of \roulette\ (except for the uncorrelated workload with $10\%$ selectivity). With views over unpartitioned datasets, we avoid the join computations but we also amplify the filtering costs. Furthermore, as Figures \ref{parcur:fig:views-cor}(c), \ref{parcur:fig:views-uncor}(c) show, these filtering costs increase with the number of query templates. Thus, if we have not first optimized the data layout, using materialized views does not help shared execution. Opposingly, when view replacement takes place in conjunction with data layout optimization, and when we plan and execute each partition separately, then the data- and filter-skipping mechanisms of Section \ref{parcur:sec:learning} reduce filtering costs and render views helpful. By eliminating both join and filtering costs, \system\ achieves a speedup of $1.6\times$ to $6.4\times$ over \roulette\ for both correlated and uncorrelated workloads. In the exception of the depicted workload in Figure \ref{parcur:fig:views-cor}(b), the join cost dominates by far the filtering costs and thus, even the unpartitioned view can yield a $1.58\times$ average speedup. Finally, Figure \ref{parcur:fig:semicor} also demonstrates the corresponding results for a semi-correlated workload, which is the best case for \system\ and the achieved speedup reaches the $12.2\times$. 

%If we only consider views (\system\ (no partitioning)), we observe that the conclusions are the exact opposite than the ones we testified before: Views favor high selectivities and join-heavy workloads. In the correlated workload, \system\ (no partitioning) is slower than \roulette\ and only becomes faster when partitioning is introduced. The same also holds for the uncorrelated workload and selectivity $1\%$. In these scan-heavy cases, scanning the materialized views and then post-filtering is more expensive than sharing execution over the base tables. Opposingly, for the join-heavy case of Figure \ref{fig:views-uncor}(b), \system\ (no partitioning) is slightly faster than \roulette\ and for a low degree of concurrency it is even faster than the partitioned \system\ (no views) version. Regardless of a scan- or join-heavy workload, the full version of \system\ outperforms \roulette\ from \textcolor{red}{X$\times$} to \textcolor{red}{Y$\times$}, and also regardless of the workload and the system we observe that the number of query templates negatively affect execution time for all systems (Figures \ref{fig:views-cor}(c), \ref{fig:views-uncor}(c)).

\begin{figure}[h]
 \centering
	\includegraphics[width=0.8\hsize]{../figures/semicor10_views.pdf}	
	\caption{Semi-correlated workload with $10\%$ selectivity on the fact table.}
	\label{parcur:fig:semicor}
\end{figure}

\textbf{Takeaway:} Materialized views accelerate shared execution only when combined with partitioning, data- and filter-skipping. By appropriately combining layout optimization and view selection, \system\ is faster than \roulette\ from $1.6\times$ to $12.2\times$ in all cases.

\subsubsection{Workload Shift}

We evaluate the impact that a workload shift has on view-based execution for a semi-correlated workload. We consider $512$ queries, which are partitioned in groups and each group targets a different range of the fact table. Each of the hot ranges consists of $5$ partitions and initially we have available materialized views that cover all the partitions of each range. As the workload shifts, we assume that some of these views are deleted by the tuner and the corresponding partitions are evaluated from scratch. 

\begin{figure}[h]
 \centering
	\includegraphics[width=0.6\hsize]{../figures/view-shift.pdf}	
	\caption{Performance degradation due to workload shift that renders more and more views obsolete}
	\label{parcur:fig:viewshift}
\end{figure}

In Figure \ref{parcur:fig:viewshift}, we assess the execution time with respect to the percentage of view misses, i.e., to the percentage of partitions that we had to re-evaluate. For the specific example, executing all partitions on top views is $3.4\times$ faster than having no views at all. However, the important thing here is that the layout optimization allows performance to gracefully degrade as more and more views are becoming obsolete and there are no abrupt transitions.

\textbf{Takeaway:} If the workload shifts smoothly, and there are no big changes in the underlying physical design, the combination of partitioning and views leads to graceful degradation of performance.

\subsection{Scalability}

To isolate the effects of concurrency, and analyze without noise the behavior of scan-heavy and join-heavy cases, all experiments up to this point are single-threaded. Therefore, to demonstrate the efficiency of \system, here, we present a scalability experiment that showcases how execution time drops as more threads are engaged.

\begin{figure}[h]
 \centering
	\includegraphics[width=0.7\hsize]{../figures/scalability.pdf}	
	\caption{Scalability with the number of threads for an uncorrelated workload of selectivity $1\%$.}
	\label{parcur:fig:scalability}
\end{figure}

Execution time drops almost linearly up to $4$ threads. However, after this point there are diminishing returns as the dataset is small and the extra threads cannot do useful work.

\begin{figure}[h]
 \centering
	\includegraphics[width=0.7\hsize,page=1]{../figures/parkour_graphs_sep.pdf}	
	\caption{Comparing different caching policies for workload A.}
\end{figure}

\begin{figure}[h]
 \centering
	\includegraphics[width=0.7\hsize,page=2]{../figures/parkour_graphs_sep.pdf}	
	\caption{Comparing different caching policies for workload B.}
\end{figure}

\begin{figure}[h]
 \centering
	\includegraphics[width=0.7\hsize,page=3]{../figures/parkour_graphs_sep.pdf}	
	\caption{Impact of using access paths for eliminating filters.}
\end{figure}

\begin{figure}[h]
 \centering
	\includegraphics[width=0.7\hsize,page=4]{../figures/parkour_graphs_sep.pdf}	
	\caption{Impact of workload shift in required filters.}
\end{figure}

\begin{figure}[h]
 \centering
	\includegraphics[width=0.7\hsize,page=5]{../figures/parkour_graphs_sep.pdf}	
	\caption{Impact of workload shift with new partially-shared query templates.}
\end{figure}


==> parcur/txt/intro-2.tex <==
Analytical applications are stressed by the combination of highly concurrent workloads and stringent response time constraints. Dashboards and reporting, machine learning applications, and monitoring utilities require the real-time processing of thousands of concurrent analytical queries. For example, dashboards in YouTube support tens of thousands of select-project-join (SPJ) queries per second, while they keep latency in the order of tens of milliseconds \cite{chattopadhyay2019procella}. Uber \cite{fu2021real} and Facebook \cite{pedreira2021interactive} also report similar use-cases, where tail latency should be in the sub-second range. Under such circumstances, where several compute-heavy queries compete for resources, computing all queries from scratch in real-time is prohibitive.

To reduce the required computations and achieve real-time responses, underlying systems take advantage of recurring patterns in the application's workload. They materialize frequently occurring intermediate results and use them to respond to most queries. However, materialization is effective only when it provides coverage for the workload; this is often impossible either due to workload shifts or insufficient space for materializing all frequent computations. Consider the following example: suppose that the workload consists of query templates

\begin{verbatim}
Q1: SELECT SUM(A.m) FROM A,B,C
    WHERE A.x=B.x and A.y=C.y 
        and A.n > 50 and A.b < k

Q2: SELECT SUM(A.m) FROM A,B
    WHERE A.x=B.x and A.n > 50
        and A.n < l
\end{verbatim}
where k, l are runtime parameters.

In case that there only enough space for one materialization, a system would cache M:

\begin{verbatim}
M: SELECT A.m, A.n, A.y FROM A,B
   WHERE A.x=B.x and A.n > 50
\end{verbatim}

Both Q1 and Q2 can be processed using M. To process Q1 using M, the system needs to filter on $A.n$ and then join with $C$, whereas to process Q2, the system needs to simply filter on $A.n$. We use the term \textit{vertical miss} to describe the additional computation for Q1 and Q2. By contrast, a new query Q3 with a filter $A.n > 4$ requires data that is absent from $M$ and therefore cannot exploit it. We use the term \textit{horizontal miss} to describe the computation for processing Q3. Both horizontal and vertical misses introduce contention when concurrency is high and thus can result in high response times. Thus, to achieve real-time responses, systems need to minimize the computations triggered by misses.

\textcolor{red}{TODO: clarify more carefully what the problem is in graph. show full reuse vs misses}

\textcolor{red}{TODO: move swiftly to Parkour}

Partial reuse \cite{gjengset2018noria, zhou2005partially, zhou2007dynamic} takes advantage of overlaps with existing materialized results. Caches focus on storing the most frequently used parts of an expression. When responding to queries, the system uses materialized computations and only recomputes non-materialized parts of the expression e.g. Q3 would process the base data only for $A.n > 4 and A.n \leq 5$. Partial reuse results in horizontal misses with tighter filters. However, it poses three key challenges. First, unless there is an efficient access method, partial reuse still has to process a large data volume. Second, they fail to exploit all reuse potential, for example between the horizontal miss and another competing materialization. Third, it introduces multiple expensive operations such as building hash-tables for joins, which jeopardise real-time responses when concurrency is high.

To minimize the impact of horizontal and vertical misses along the lines of the three chanllenges, we propose Parkour: a system that efficiently exploits materialization to minimize computation for misses. Parkour builds a novel execution method based on partitioning and work-sharing. On the one hand, partitioning decomposes reuse into independent reuse decisions: in each partition, is either fully covered by the materializations or results in a full miss. Then, competition between materializations turns into synergy as they cover different data partitions. Furthermore, partitioning contains horizontal misses within a small subset of the data, thus reducing the performance penalty. On the other hand, work-sharing eliminates common computation between both horizontal and vertical misses computed within each partition's boundaries. As a result, the system amortizes the computations and can provide fast response times despite misses.

\textcolor{red}{TODO: add example in para below}

Evidently, reuse decisions are not orthogonal to sharing decisions. As the cost of vertical misses is amortized, the most cost-effective reuse decision depends on the potential for sharing. Rather than filtering separate materializations, queries may benefit from using a common materialized sub-expression, increasing the potential for sharing common filters and joins. The correct decision depends on the data and queries that process the partition and thus requires taking the sharing potential into account.
To effectively combine materializations and sharing, Parkour uses an reinforcement learning algorithm that adapts the interaction between the two for the specific workload. The algorithm is online and adapts the query plans at runtime, thus avoiding fragile heuristics that depend on inaccurate estimates.

By combining partial reuse and sharing, Parkour reduces miss overhead but also affects prior assumptions about materializations as well. Using work-sharing affects both the benefit of materializing an expression and the miss cost in case the system chooses not to materialize. Furthermore, the data layout is critical for the effectiveness of reuse. The data layout needs to support efficient access to data, such that expensive shared filters are avoided. Based on historical access patterns, Parkour introduces a sharing-aware cache policy that chooses both what to materialize and how to store it in order to avoid redundant accesses and filters.

\textbf{The contributions of this work are the following}:

\begin{itemize}
    \item We propose \system: a framework that efficiently handles concurrent compute-heavy workloads, regardless of the query batch size. By combining partial materialization and sharing-aware execution, \system{} both improves cache utilization and reduces miss penalties. Consequently, \system{} provides real-time responses even for highly-concurrent compute-heavy queries.
    \item Introducing materialized views in shared query plans is not straightforward. We show that naive injection can lead to considerable slowdowns of execution. Instead, we propose that views should be always accompanied by data layout optimizations that enable data skipping, and filter skipping.
    \item Deciding which views to use and when in a shared executor defines an intractable optimization problem. To avoid inaccurate heuristics, we design a reinforcement learning algorithm that continuously alternates among different access paths until it learns how views and sharing can optimally cooperate. 
\end{itemize}

==> parcur/txt/intro.tex <==
% Apart from the ever exploding data volume, large organizations are also stressed by the combination of highly concurrent workloads and stringent response time constraints. Dashboards and reporting, machine learning applications, and monitoring utilities require the real-time processing of thousands of concurrent analytical queries. 

% For example, dashboards in YouTube support tens of thousands of select-project-join (SPJ) queries per second, while they keep latency in the order of tens of milliseconds \cite{chattopadhyay2019procella}. Similarly, the analytical processing infrastructures of Uber \cite{fu2021real} and Facebook \cite{pedreira2021interactive} also strive to maintain tail latency in the sub-second range.

\textcolor{red}{Update intro to match scope of paper. Now we are focusing on caching so we need to tone down selections}

Large organizations are stressed by the combination of highly concurrent workloads and stringent response time constraints. Dashboards and reporting, machine learning applications, and monitoring utilities require the real-time processing of thousands of concurrent analytical queries. For example, dashboards in YouTube support tens of thousands of select-project-join (SPJ) queries per second, while they keep latency in the order of tens of milliseconds \cite{chattopadhyay2019procella}. Uber \cite{fu2021real} and Facebook \cite{pedreira2021interactive} report similar use-cases, where tail latency should be in the sub-second range.

\textcolor{red}{Moreover, many of these workloads are selective and only touch a small fraction of the data \cite{chattopadhyay2019procella}. To achieve low latency and avoid costly full scans, systems usually employ indexing, partitioning and materialization that permit selective accesses, data skipping, and prune computation. However, as concurrency increases, processing costs dominate data-accesses and become the bottleneck of execution. Assuming sufficiently enough resources, we could reduce contention and preserve low latency by replicating the data and scaling-out the execution.}

% The most straightforward solution when serving latency-critical queries is to prune computation and avoid expensive data accesses by having available an elastic memory-resident cache \cite{nishtala2013scaling} and aggressively using materialized views for \emph{hot} sub-expressions. However, this entails several drawbacks: (i) DRAM is still a scarce resource and caching everything is not a viable option, (ii) pre-fetching hot data by predicting the workload is an error-prone process that leads to expensive cache-misses, and (iii) from a degree of concurrency and onward, the processing costs dominate data-accesses, leaving the memory-bus under-utilized and rendering even the post-filtering of views prohibitively expensive. By selectively materializing the most beneficial views \cite{kalnis2002view}, or by building indices that accelerate selective workloads, we can bypass points (i) and (ii), but (iii) remains to be a problem: \emph{even with the right physical design at hand, concurrency can render processing unaffordable}.

\begin{figure}[t]
 \centering
	\includegraphics[width=0.7\hsize]{../figures/motivation.pdf}	
	\caption{Conceptual graph showing the effect of concurrency on query latency when various techniques are used.}
	\label{parcur:fig:motivation}
\end{figure}

By amortizing both data-access and processing costs across multiple different queries, \emph{sharing} bounds latency and offers a more resource-efficient alternative for high-concurrency workloads. However, the shared execution of a small or medium query batch can still be significantly slower than the query-at-a-time execution when indices/views are available. Moreover, even for large batches, sharing does not take into account query access patterns and eagerly spreads overheads across all data.

%eagerly spreads overheads across all data regardless of the query access patterns. 

This is better explained in Figure \ref{parcur:fig:motivation}, which qualitatively illustrates how the query latency of each technique is expected to be affected by concurrency. Views and indices provide instant responses for a low or mediocre query-load, but latency sharply increases with the concurrency and soon becomes unbounded \cite{kester2017access}. Typical sharing approaches always require a full-scan over the data, and this scan cost is the lower bound for latency. Adding more queries to the system slightly affects the response time; the scan cost remains almost the same and an overhead is added due to the computation of non-shared sub-expressions, query-set manipulation and routing of results \cite{sioulas2021scalable}. Despite its robust behavior, the full scan of sharing is significantly more expensive than the selective access that an index or view can provide, and thus hinders interactivity.

This work is motivated by two key-observations: First, there is no clear winner in concurrent analytics, but the degree of concurrency defines a design space split in two regions: region \circled{I} where physical design-aware query-at-a-time execution is the strategy of choice, and region \circled{II} where sharing dominates. Existing systems take static decisions and operate only in one of the two regions, missing opportunities for a plethora of workloads.
%Selecting the most advantageous execution mechanism is a responsibility of the query optimizer, which is also stressed by concurrency: sharing-aware optimization (SWO) is an NP-hard problem \cite{giannikis2014shared, giannikis2012shareddb}, and thus heuristics that usually lead to sub-optimal plans are employed. 
Second, and most important, we acknowledge that there is no technique available for providing real-time responses in region \circled{II}. 

To deal with the aforementioned problems, we propose \emph{\system}: a system that efficiently covers the whole space in a unified way. To increase interactivity for highly concurrent workloads, \system{} builds a novel execution mechanism based on the following paradoxical observation: Although both sharing and views/indices can become too expensive under high query-load, by exposing the physical design to the shared executor, latency drops. Then, having appropriate execution mechanisms for the whole spectrum, it uses a reinforcement-learning (RL) algorithm that blurs the boundaries between optimization and execution, and adapts the query plans at run-time in order to minimize the query batch execution time. 

By making sharing \emph{physical-design-aware}, we avoid the full scan over the data, but we face the following challenge: \emph{Queries with shared input tables do not necessarily require the same indices or the same set of views}. This creates a bidirectional dependency between physical design selection and sharing. On the one hand, we should decide on a physical design that favors individual queries, and at the same time amortizes costs based on a given global plan. On the other hand, sharing-aware optimization must identify the extra opportunities that the existing physical design exposes and consider a larger space of available execution plans. As both sharing-aware optimization and physical design selection already have an exponential complexity \cite{gupta1997selection, giannikis2014shared}, their co-optimization defines an intractable problem.

To make it manageable, we decouple physical design selection and sharing-aware optimization.
%, and we formulate two separate problems where the output of each one is fed to the input of the other through a feedback loop. 
Following the trend of scan-oriented analytical systems, our physical design selection includes: (i) data-layout selection \cite{yang2020qd}, (ii) zone-map indices for data skipping \cite{graefe2009fast}, and (iii) view materialization. Execution-wise, our approach relies on the ideas of \emph{partially stateful systems} \cite{zhou2005partially, gjengset2018noria, yang2021flexpushdown}, where there are multiple access paths available for each query. By applying the right data-layout based on the workload and using data-skipping, we decompose batched execution into many independent sub-problems (one for each partition), and we select a different access path for each of them. Then, as already mentioned, the sharing-aware optimization of selecting access paths for each partition takes place through a reinforcement learning algorithm that is scalable and chooses execution plans of low latency.

\textbf{The contributions of this work are the following}:

\begin{itemize}
    \item We propose \system: a framework that efficiently handles concurrent selective workloads in a unified way, regardless of the query batch size. By co-optimizing physical design and sharing-aware execution, \system{} sustains the load and provides real-time responses even for highly concurrent adversarial cases.
    \item Introducing materialized views in shared query plans is not straightforward. We show that naive injection can lead to considerable slowdowns of execution. Instead, we propose that views should be always accompanied by data layout optimization, data skipping, and filter skipping.
    \item Deciding when and which views to use in a shared executor defines an intractable optimization problem. To avoid inaccurate heuristics, we design a reinforcement learning algorithm that continuously alternates among different access paths until it learns how physical design and sharing can optimally cooperate. By using this algorithm, \system\ outperforms a state-of-the-art work-sharing system \cite{sioulas2021scalable} by $1.6\times$ to $12.2\times$. 
\end{itemize}





==> parcur/txt/learned-execution.tex <==
\section{Sharing- and Physical Design-Aware Execution }
\label{parcur:sec:learning}

\system\ exploits the physical design to reduce computation. Specifically, it uses the data layout to optimize data accesses and restrict the number of queries that access each partition, and the views to eliminate recurring computations. 
%Hence, within each data partition, the global plan is stripped down to the absolutely necessary computations.

To render shared execution aware of the physical design, we enhance existing approaches in two levels: First, we use data- and filter skipping to identify the queries that access each partition and to optimize selections. Second, we design a view- and sharing-aware framework that selects a different access path for each partition. 
%We describe data skipping in Section \ref{parcur:data-skipping}, and present our optimization algorithm in Section \ref{parcur:view-aware-sharing}.

\subsection{Shared Execution Model}

\textcolor{red}{TODO: Move to background.}

\system\ uses two techniques to efficiently process a batch of queries: (i) the global plan and (ii) the Data-Query model.

The global plan is a DAG of relational operators that, in each of its roots, produces the results of the participating queries. Each node of the DAG corresponds to an operator that processes tuples for one or more queries and broadcasts results to one or more parent operators. By processing each operator once for the whole batch, the system shares work across queries and reduces the overall processing time.

The Data-Query model abstracts away predicates and allows merging queries with different selection operators into a common global plan. Specifically, the Data-Query model annotates each tuple with a \textit{query-set} that indicates to which queries the tuple contributes. Then, specialized relational operators process both the actual tuples and the query-sets in order to maintain the correctness of intermediate results. 
%Specifically, the Data-Query model annotates tuples with \textit{query-set} whose predicates they satisfy. Specialized relational operators process the query-set so that they produce the correct query-sets for intermediate results.
The advantage of this representation is that: (i) the global plan can share work on tuples that are common across some but not all queries, and (ii) the operators can immediately drop tuples that do not belong to any query. In \system, query-sets are represented as bitsets where the $i_{th}$ bit represents the $i_{th}$ query e.g. a bitset 0101 means that the tuple belongs to queries 0 and 2. All operators rely on bitset operations and follow the implementation used in \cite{sioulas2021scalable}.

\subsection{Data Skipping}
\label{parcur:data-skipping}

\system\ uses the data layout to identify the queries that each partition processes. By doing so: (i) it reduces the number of queries in the per partition global plan, and (ii) it completely skips some partitions. For selective correlated workloads, where all queries only access and process a few hot partitions, data skipping drastically reduces the batch response time.

As Qd-tree uses query filtering predicates to apply cuts in the data space, each partition's boundaries are defined by a set of predicates. A query $q$ skips a partition $p$ if the data region defined by $q$'s predicates does not overlap with $p$. For example, the query \texttt{\Verb"SELECT COUNT(*) FROM T WHERE x > 8"} will skip partition $5 \leq x < 7$, as the two ranges do not overlap. For each partition, \system\ finds the set of queries that cannot be skipped and forms a global plan that only applies to the specific partition.

To compute the query-set of each partition, we combine zone maps \cite{graefe2009fast} with predicate indexing \cite{madden2002continuously}. Zone maps express the partition's predicates by storing min-max statistics for each attribute. Predicate indexing organizes and stores all the query predicates on a per attribute basis, and returns the set of queries that are satisfied for each value of the attribute. 

Our implementation stores the query-set for each range in the attribute's domain. We extend predicate index with range lookup; we retrieve the set of predicates that are satisfied by at least one value in the min-max range. For this computation, we identify the range for the min value and scan ranges of increasing values until the range that contains the max value. The result is the union of the queries in the scanned ranges.

During table scan, \system\ performs the satisfiability test for each partition. If the resulting query set is empty, no processing is required and the partition is skipped. Otherwise, we process the partition for the eligible queries in a vector-at-a-time fashion. In this manner, global plans are specialized to the access patterns of the batched queries.

\subsection{Filter Skipping}
\label{parcur:filter-skipping}

\system\ also uses the data layout to identify which predicates hold for all tuples of each partition. Consequently, it avoids re-computing partition-wide predicates, and only evaluates predicates that differ from tuple to tuple. For example, the predicate of query \texttt{\Verb"SELECT COUNT(*) FROM T WHERE x > 4"} is true across the whole partition $5 \leq x < 7$ and, thus, it is redundant to evaluate it for every tuple. By contrast, the predicate of query \texttt{\Verb"SELECT COUNT(*) FROM T WHERE x > 6"} is true for only some of the partition's tuples and requires processing on a tuple-by-tuple basis. Hence, it drastically reduces costs in filter-heavy global plans, which are common when queries are answered by directly filtering materialized views.

To skip all but the absolutely necessary filters, \system\ identifies which queries have ambivalent predicates, i.e., they are satisfied by some of the partition's tuples and not satisfied by others. To compute such queries, we exclude queries that either do not process the partition or process all tuples in the partition. The data skipping mechanism of Section \ref{parcur:data-skipping} identifies the former. For the latter, we again combine zone maps with predicate indexing. During each range lookup, we compute the intersection of queries in the scanned ranges, which are queries satisfied across the predicate index. Then, by taking the intersection of satisfied queries across all predicate indices, we compute the queries that process the whole partition. After excluding statically evaluated queries, \system\ focuses only on the ambivalent predicates.

\subsection{Learning Execution Plans}
\label{parcur:view-aware-sharing}

\textcolor{red}{This subsection is very long, maybe we need to fragment it to pieces}

For each partition, \system\ optimizes and processes a batch of (possibly different) qualifying queries. To minimize response time, when optimizing each of these batches, it also considers the available views -- that the tuner has created -- and multiple work-sharing options. The outcome of this process is a partition-scoped global plan that simultaneously takes advantage of both materialized views and sharing opportunities. 

This optimization problem differs both from query-at-a-time view selection and sharing-aware optimization. Query-at-a-time approaches miss the impact of sharing, whereas first creating a sharing-aware optimal plan and then replacing materialized sub-expressions leads to sub-optimal results. View selection and sharing-aware optimization are tightly coupled and constitute a unified problem, which we formally define:

\begin{defn}[\vswo]
\label{parcur:def:vswo}
\emph{Given a set of materialized views $V$ and a batch of queries $Q$, the VSWO problem requires the construction of a global plan $G$ that optimally uses $V$ and exploits sharing opportunities in order to minimize the execution time of $Q$.}
\end{defn}

\textcolor{red}{Notes for below: even normal QO is exponential, also now we do two-phase solution.}

As the complexity of \vswo\ is exponential, optimally solving it at runtime is prohibitive. Even solving the two problems separately in two phases (i.e., view selection and then sharing-aware optimization, or sharing-aware optimization and then view selection) either results in a sub-optimal solution or in enumerating a very large number of sub-problems to solve in two phases.
For this reason, we follow the adaptive sharing-aware optimization paradigm, which was pioneered by the state-of-the-art \roulette\ system \cite{sioulas2021scalable}. Through a reinforcement learning (RL) mechanism, that balances exploration and exploitation, \roulette\ produces efficient global plans, while exposing a scalable optimization process. However, \roulette\ is view- and layout agnostic. \system\ addresses the generalized \vswo\ problem by a similar RL-based learning algorithm that continuously improves the combination of selected views and sharing decisions.

This section presents \system's algorithm for solving the \vswo\ problem. We first present an overview of \roulette, we then describe the abstractions that enable a solution for the generalized \vswo\ problem and finally, we formulate an RL-based solution.

\subsubsection{Adaptive Sharing-aware Optimization}
\label{parcur:adaptive-opt} 

Throughout the lifetime of a query batch, \roulette\ continuously optimizes the global plan. Query execution is split into episodes, where each episode corresponds to the processing of a single data vector and is the quantum for planning and execution. Thus, each data vector is executed by a possibly different global plan. By using the intermediate cardinalities observed during the episode as feedback, \roulette\ learns the cost of various sub-plans and exploits this knowledge to produce increasingly efficient global plans. 

To produce a new plan, \roulette\ follows a bottom-up approach. At each step, starting from the episode's input vector, it adds an operator to the plan. The possible options for this new operator are called \emph{candidates}. If after adding a new operator $o_i$, the resulting sub-expression covers only a subset $S$ of the queries $Q$, the decision results in \emph{divergence}: $S$ is processed by $o_i$, while $Q\setminus S$ is planned independently. Hence, each decision affects the sharing decisions for all downstream operators. For this reason, \roulette\ each time decides which operator to add based on the total estimated cost of all downstream operators (including both branches in case of divergence).

Since the quality of learning depends on the cumulative costs of downstream operators, \roulette\ uses Q-learning. RL algorithms naturally fit the problem of learning cumulative costs. \roulette\ specializes Q-learning for sharing-aware optimization: (i) it exploits the independence between branches, that divergence creates, and (ii) it takes advantage of the proportionality between the input size and the observed cost. \roulette\ expresses the peculiarities of sharing as a new update rule in Q-learning that improves the estimates of aggregate downstream costs for each candidate operator. 

\textcolor{red}{TODO: Update with new simpler and extensible formulation.}

\subsubsection{Incorporating View-selection}
\label{parcur:incorporating-views}

In contrast to \roulette, the global plans that \system\ produces can also use \textcolor{red}{materialized views}. In this section, we show how we can efficiently explore the search space of the \vswo\ problem, optimize the total cost and prune out globally sub-optimal solutions.

\system\ also builds the global plan in a bottom-up fashion and adds a new operator at a time. However, when the sub-expression of the new operator matches an existing view, the learning algorithm has an extra option: to use the view for the computation of all downstream operations. For example, in Figure \ref{parcur:fig:virtops}(a), we ingest a vector from relation $R$ and the RL algorithm decides to first insert a join with $S$, and then a join with $T$. At this point, as the materialization of $R \Join S \Join T$ is available, the algorithm should be also able to replace it with the materialized view.

A technical problem at this point is that an episode gets as input a vector from the base data. In case the algorithm decides to use the view, it should know which part of the view corresponds to the specific input vector, and directly scan and apply filters to the view-vector. For this purpose, we maintain an index that is built during view materialization. This index keeps the lineage of intermediate results, so that we can associate them with the corresponding input vectors. Following this approach, the evaluation of the plan starts from the materialized view and all preceding computations are avoided. Therefore, incremental planning can produce both view- and sharing-aware global plans.

\begin{figure}[h]
\begin{tabular}{@{}l@{}l}
\begin{minipage}{0.5\hsize}
    \centering\includegraphics[width=10pc]{../figures/rljoins.pdf}\\
        \centering {\footnotesize(a) RL with no views}
        \end{minipage}
        &
    \begin{minipage}{0.5\hsize}
\centering\includegraphics[width=10pc]{../figures/vops.pdf}\\
    \centering {\footnotesize(b) virtual operators}
    \end{minipage}
\end{tabular}
\caption{\label{parcur:fig:virtops} View replacement and virtual operators.}
\end{figure}

In reinforcement learning terms, adding a new operator to the plan signifies an \emph{action}, and each action is associated with a \emph{reward} (i.e., the operator's cost). For example, see Figure \ref{parcur:fig:virtops}(a). However, in \system, a view-replacement action can nullify the effect of a past action. In Figure \ref{parcur:fig:virtops}(b), if we decide to use the $R \Join S \Join T$ view, then we should cancel the rewards for $R \Join S$ and $R \Join S \Join T$ since these joins will never take place and we should give a reward from scanning and filtering the view. Therefore, in order to pay rewards only once, the rewards have to be delayed until we ensure that no other view replacement will occur. In that case, the RL state needs to carry extra information about the pending rewards. Tracking pending rewards results in backward dependencies on past actions and significantly expands the state space of the learning algorithm.

To facilitate learning, we convert backward to forward dependencies by introducing \emph{virtual operators}:

\begin{defn}[Virtual Operator]
\emph{A virtual operator is a commitment that all queries that use this operator will also use a view later in the downstream path of the global plan.}
\end{defn}

Thus, the virtual operator acts as a marker that signifies that all subsequent operators up to the first encountered view must get a zero reward (as the view will cancel the rewards either way). Now, if a non-virtual operator results in a view replacement for all queries, the sub-plan is sub-optimal compared to an equivalent plan that starts with a virtual operator, and therefore will be pruned out by exploration.

To further analyze the use of virtual operators and to explain our learning mechanism, we introduce some additional terminology and notation:

\begin{defn}[Dependency Graph]
\emph{The dependency graph of a set of operators $O$ is
defined as the complete graph $K_{| O |}$ if $O$ comprises selections and
as $G = (V , E)$ with $(e_1, e_2) \in E \text{ iff } \\ e_1 \Join e_2 \in O$ if $O$ comprises joins}.
\end{defn}

\begin{defn}[Lineage]
\emph{Let $O$ a set of operators with dependency graph
$G(O)$. A subset $\mathcal{L} \subset O$ is defined as a \emph{lineage} iff the induced subgraph $G(O)[\mathcal{L}]$ is connected. The set of lineages is $\mathcal{L}^{\ast}$}.
\end{defn}

\begin{defn}[Query-set]
\emph{The query-set $Q_o$ of an operator $o$ is defined as the set of queries that contain $o$}.
\end{defn}

\begin{defn}[Virtual Vector]
\emph{A virtual vector is defined as a pair $(\mathcal{L}, Q)$}.
\end{defn}

Virtual operators come with a prerequisite: the corresponding commitment needs to be \emph{enforceable}, i.e., the view needs to cover all queries that use the new sub-expression. We define the \emph{enforceability} test as follows: For each view $v$, we define a coverage query set $Q_v = \{ q_i | O_v \subset O_{q_i} \}$ where $O_v$ are the operators in $v$'s sub-expression and $O_{q_i}$ are the operators in $q_i$'s expression. Let $(\mathcal{L}, Q)$ be the virtual vector at some planning step. A virtual operator results in a downstream plan that can use views for all queries in $QV(\mathcal{L}, Q) = Q \cap (\cup_{v \in V | \mathcal{L} \subset v} (Q_v))$. If $QV(\mathcal{L}, Q)$ is empty, no virtual operator can be added, and the commitment is not enforceable.

In case the commitment is enforceable, we apply it with the following mechanism: After choosing a virtual operator, planning can choose only virtual operators in the downstream plan until a branch reaches a sub-expression covered by the view. Then and only then, the view replacement occurs and the commitment ends. In Figure \ref{parcur:fig:virtops}, the green circles denote virtual operators which we assume to be enforceable. Initially, the learning algorithm decided to insert the virtual operator \circled{$\Join S$} in the plan and received a zero reward. As there is not any materialized view for the $R \Join S$ subexpression, the optimizer must mandatory select another virtual operator and \circled{$\Join T$}. Now, the $R \Join S \Join T$ subexpression matches an available view, and the algorithm can choose between an actual or a virtual operator\footnote{In the specific example, as there is no materialized view that expands $R \Join S \Join T$ the algorithm can only select an actual operator}. If an actual operator is selected, then all nodes between the first encountered virtual operator and the current actual operator are replaced by the corresponding view.

Adding virtual operators into planning expands the search space. Apart from the view-oblivious plans that \roulette\ generates, by designing a Q-learning-based algorithm that predicts which operators (virtual or not) minimize the estimated cost, \system\ also explores view-aware sharing options and solves the \vswo\ problem.

\subsubsection{Cost propagation}
\label{parcur:combined-cost} 

To successfully learn cumulative costs in a global plan that uses views, virtual operators need to propagate costs to upstream operators. Therefore, for the intermediate states leading up to the view replacement, the algorithm needs to learn estimates of downstream cumulative costs. However,  virtual operators do not process data and do not have known input and output cardinalities. Thus, they cannot provide normalized cardinality as typically in \roulette.

We address normalization by introducing \emph{virtual states}. We call \emph{virtual} the states that exist between the first encountered virtual operator and the view replacement. Virtual states have an input cardinality equal to $1$. Hence, if a virtual operator leads to a virtual state, then its output cardinality is $1$, otherwise it is the cardinality that occurs after the view replacement by scanning the corresponding view. Using virtual states, costs that are downstream for different view replacements can be both accumulated when divergence happens and compared in order to find the most efficient view replacement.

\subsubsection{Reinforcement Learning for \vswo}
\label{parcur:formulation} 

The use of virtual operators and states affects the formulation of the Markov Decision Process (MDP) that \roulette\ employs for optimization. 

%\system\ addresses the view and sharing-aware optimization problem by introducing virtual operators and virtual states. The additions affect the Markov Decision Process formulation of the problem.

\textbf{State:} State contains all the required information for decision-making. In \roulette, singular decisions require knowledge of the cardinality ($n$), the lineage ($\mathcal{L}$) and the query-set ($Q$) of the corresponding step. Divergent steps are combined together into a stack of $((n, \mathcal{L}, Q):tail)$ triplets. We denote stacks as $(head:tail)$.

%\textbf{State:} State contains all the required information for decision-making. In RouLette, singular decisions already require the cardinality, lineage and query-set of the corresponding step. Divergent steps are combined together into a stack of $(n, L, Q)$ triplets.

In \system, decision-making requires additional information for the commitments of virtual operators. A commitment implies a \emph{virtual state} which mandates: (i) all queries to be answered from a view, and (ii) from this point and onward, only virtual operators are eligible actions. To account for the commitments, \system\ enriches the state of \roulette\ with the boolean $c$ value, which is is \emph{true} if the state is virtual and \emph{false} otherwise. Hence, state becomes a stack of quadruples $((n, \mathcal{L}, Q, c):tail)$. 

%In \system, decision-making requires additional information for commitment. A commitment implies that the state is virtual, thus a) all queries need to be answered from a view, and b) only virtual operators are eligible actions. Hence, state is a stack of $(n, L, Q, c)$ where $c$ is a boolean value -- true if the state is virtual and there is a commitment, otherwise false.

\textbf{Actions:} Our formulation for actions separates actual and virtual operators. Thus, every decision is an $(a, v)$ pair, where $a$ is the operator to be added in the plan, and $v$ a boolean value that indicates whether $a$ is virtual or not.
Thus, actions for actual operators are represented as:
$$
A^A((n, \mathcal{L}, Q, c):tail) = \{ (a, false) | a \in cand(\mathcal{L}, Q) \}
$$
whereas actions for virtual operators as:
\begin{equation*}
\begin{split}
A^V((n, \mathcal{L}, Q, c):tail) = \{ (a, true) | a \in cand(\mathcal{L}, Q)\  \\ \text{ and } Q \cap \cup_{v \in V | \mathcal{L} \subset v} (Q_v) \neq \emptyset \}
\end{split}
\end{equation*}
Please note that adding a virtual operator requires the corresponding commitment to be enforceable.
Then, the idea is that when we are in a non-virtual state, the algorithm can add either an actual or a virtual operator, and this is formally represented as:
\begin{equation*}
\begin{split}
A((n, \mathcal{L}, Q, false):tail) = A^A((n, \mathcal{L}, Q, c):tail) \\ \text{ } \cup A^V((n, \mathcal{L}, Q, c):tail)
\end{split}
\end{equation*}
whereas when we are in a virtual state we can only add virtual operators and we denote it as:
$$
A((n, \mathcal{L}, Q, true):tail) = A^V((n, \mathcal{L}, Q, c):tail)
$$

% \textbf{Actions:} The formulation separates actual and virtual operators. Thus, every decision is a pair $(a, v)$ where a is the operator and v is a boolean value -- true if it is a virtual operator else false.
% We represent actions for actual operators as 
% $$
% A^A((n, L, Q, c):tail) = \{ (a, false) | a \in cand(L, Q) \}
% $$
% and the virtual operators as
% $$
% A^V((n, L, Q, c):tail) = \{ (a, true) | a \in cand(L, Q)\ and\ Q \cap \cup_{v \in V | L \subset v} (Q_v) \neq \emptyset \}
% $$
% Then, the available actions are
% $$
% A((n, L, Q, false):tail) = A^A((n, L, Q, c):tail) \cup A^V((n, L, Q, c):tail)
% $$
% and
% $$
% A((n, L, Q, true):tail) = A^V((n, L, Q, c):tail)
% $$

\textbf{Transitions:} In case of an actual operator, transitions work in the same way as in \roulette: they replace the top of the stack with one or two new elements, depending on whether there is divergence. If there is no divergence:
$$((n_{in}, \mathcal{L}, Q, false):tail) \xrightarrow{(a, false)} ((n_{out}, \mathcal{L} \cup a, Q, false):tail)$$
While in the case of divergence, transition becomes:
\begin{gather*}
        ((n_{in}, \mathcal{L}, Q, false):tail) \xrightarrow{(a, false)} \\ ((n_{out}, \mathcal{L} \cup a, Q \cap Q_a, false):(n_{div}, \mathcal{L}, Q-Q_a, false):tail)
\end{gather*}

In case of a virtual operator, and when view replacement does not occur immediately, one branch might result in a virtual state. Therefore, if there is no divergence:
$$((n_{in}, \mathcal{L}, Q, c):tail)\xrightarrow{(a, true)} ((n_{out}, \mathcal{L} \cup a, Q, c_{out}):tail)$$
Otherwise:
\begin{gather*}
        ((n_{in}, \mathcal{L}, Q, c):tail) \xrightarrow{(a, true)} \\ 
        (n_{out}, \mathcal{L} \cup a, Q \cap QV(\mathcal{L} \cup a,Q), c_{out}): \\ (n_{div}, \mathcal{L}, Q-QV(\mathcal{L} \cup a,Q), c):tail)
\end{gather*}

If $\mathcal{L} \cup a$ corresponds to an available view, $c_{out}$ is \emph{true} and $n_{out}$ is the size of the scanned view-vector, otherwise $c_{out}$ is \emph{false} and $n_{out}$ equals to $1$. In case $c$ is \emph{true}, then $n_{div}$ is $1$.

%If $\mathcal{L} \cup a$ corresponds to an available view, $c_{out}$ is true and $n_{out}$ is the size of the vector scanned from the view, otherwise $c_{out}$ is false and $n_{out}$ is 1. Also, if $c$ is true, then $n_{div}$ is 1.

\textbf{Rewards:} Each action results in a reward. For an actual operator, the rewards are the same as in \roulette. If there is no divergence, the reward is:

\begin{gather*}
R((((n_{in}, L, Q, c):tail), (a, false)) = \\
\begin{cases}
\text{$- c_a(n_{in}, n_{out})$} &\quad\text{if no divergence}\\
\text{$- c_a(n_{in}, n_{out}) - c_{\sigma}(n_{in}, n_{div})$} &\quad\text{otherwise}\\
\end{cases}
\end{gather*}

For virtual operators, the reward is always zero: 

$$
R(((n_{in}, L, Q, c):tail), (a, true)) = 0
$$

\textbf{Specialization:} \roulette\ uses \emph{proportionality} and \emph{independence} to reduce the state space size and to improve Q-learning's efficiency. The same principles apply to \system\ as well.
%We specialize Q-learning for our use case and learn Q-values for $(n, \mathcal{L}, Q, c)$ tuples. \textcolor{red}{Algorithm Y} presents the pseudocode for both choosing the next operator to process, and for updating the Q-values using proportionality and independence.

==> parcur/txt/main.tex <==
\input{parcur/txt/intro-3.tex}

%\input{parcur/txt/related}

\input{parcur/txt/motivation}

%\section{Introduction}
%\label{sec:intro}
%\input{intro}

%\section{Problem Formulation}
\input{parcur/txt/parcur.tex}
\input{parcur/txt/physical-design}
\input{parcur/txt/learned-execution-2}
\input{parcur/txt/implem.tex}
\input{parcur/txt/experiments-2}

\section{Summary}
\label{parcur:sec:conclusions}
\input{parcur/txt/conclusions}

